RoboDojo: A Unified Sim-and-Real Benchmark for Comprehensive Evaluation of Generalist Robot Manipulation Policies

Generalist robot manipulation policies have advanced rapidly, yet existing benchmarks remain limited in systematically evaluating their capabilities. Many rely on simple, short-horizon, or skill-narrow tasks with limited capability coverage, and are often conducted only in simulation or only in the real world. Simulation enables scalable feedback but misses physical deployment challenges, while real-world evaluation is costly, time-consuming, and difficult to reproduce. We introduce RoboDojo, a unified sim-and-real benchmark for comprehensive evaluation of generalist robot manipulation policies. RoboDojo includes 42 simulation tasks and 18 real-world tasks covering diverse and complementary manipulation capabilities. The simulation benchmark evaluates five dimensions: generalization, memory, precision, long-horizon execution, and open-vocabulary instruction following, while the real-world benchmark exposes policies to challenging physical-world deployment conditions. RoboDojo supports scalable evaluation through heterogeneous parallel simulation in Isaac Sim and provides RoboDojo-RealEval, a reproducible real-world evaluation system with remote cloud access, standardized hardware, scene reset, evaluation protocol, and deployment interface. Together with XPolicyLab, policies can be integrated once and evaluated across simulation and real-world settings with minimal adaptation. We integrate 30 policies into XPolicyLab and evaluate them on RoboDojo, establishing a public leaderboard and systematic analysis of current policy performance. The website is available at http://robodojo-benchmark.com/.

==> sec/6.9_open_source.tex <==
\section{Open-Source}
\label{sec:open-source}

==> table/eval_result_details.tex <==
% =========================================================
\subsection{A1}
\label{part:a1}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.10 & 0 & 0.00 & 0 & 0.10 & 0 ±0 & 0.07 ±0.05 \\
fold\_clothes & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
hang\_mugs & 0 & 0.60 & 0 & 0.30 & 0 & 0.00 & 0 ±0 & 0.30 ±0.30 \\
make\_toast & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pack\_objects\_into\_box & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_bowls & 0 & 0.00 & 2 & 2.90 & 0 & 0.90 & 1 ±1 & 1.27 ±1.45 \\
store\_laptop\_and\_headphones & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.80 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.40 ±0.40 \\
deposit\_coin & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fasten\_screws & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_key & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_tubes & 0 & 0.00 & 0 & 0.00 & 0 & 0.80 & 0 ±0 & 0.27 ±0.40 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_egg\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 6.50 & 0 & 7.00 & 0 & 10.00 & 0 ±0 & 7.83 ±1.75 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
put\_bottles\_into\_dustbin & 0 & 3.30 & 0 & 1.70 & 0 & 2.90 & 0 ±0 & 2.63 ±0.80 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.20 & 0 & 0.00 & 0 & 0.10 & 0 ±0 & 0.10 ±0.10 \\
match\_and\_pick\_from\_conveyor & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.0 & 0.27 & 0.0 & 0.29 & 0.0 & 0.35 & 0 ±0 & 0.31 ±0.04 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{ACT}
\label{part:act}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fold\_clothes & 0 & 0.80 & 0 & 0.80 & 0 & 0.00 & 0 ±0 & 0.53 ±0.40 \\
hang\_mugs & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_toast & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pack\_objects\_into\_box & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_liquid\_into\_cup & 6 & 6.00 & 8 & 8.00 & 6 & 6.00 & 7 ±1 & 6.67 ±1.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.30 & 0 ±0 & 0.10 ±0.15 \\
stack\_bowls & 0 & 0.60 & 0 & 0.00 & 0 & 0.60 & 0 ±0 & 0.40 ±0.30 \\
store\_laptop\_and\_headphones & 0 & 0.00 & 0 & 1.60 & 0 & 0.00 & 0 ±0 & 0.53 ±0.80 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 5.00 & 0 & 4.60 & 0 & 5.00 & 0 ±0 & 4.87 ±0.20 \\
deposit\_coin & 0 & 0.40 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
fasten\_screws & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_key & 0 & 1.20 & 0 & 0.60 & 0 & 1.20 & 0 ±0 & 1.00 ±0.30 \\
insert\_tubes & 0 & 1.60 & 0 & 0.00 & 0 & 0.80 & 0 ±0 & 0.80 ±0.80 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.30 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.10 ±0.15 \\
fill\_egg\_holder & 0 & 0.20 & 0 & 0.60 & 0 & 0.20 & 0 ±0 & 0.33 ±0.20 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_kong & 8 & 8.00 & 8 & 8.00 & 6 & 6.00 & 7 ±1 & 7.33 ±1.00 \\
organize\_table & 0 & 0.00 & 0 & 0.00 & 0 & 0.50 & 0 ±0 & 0.17 ±0.25 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.40 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.40 ±0.00 \\
put\_bottles\_into\_dustbin & 0 & 4.40 & 0 & 6.40 & 0 & 5.70 & 0 ±0 & 5.50 ±1.00 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 2 & 9.40 & 0 & 6.50 & 0 & 8.50 & 1 ±1 & 8.13 ±1.45 \\
imitate\_sorting\_sequence & 0 & 0.10 & 0 & 0.00 & 0 & 0.20 & 0 ±0 & 0.10 ±0.10 \\
match\_and\_pick\_from\_conveyor &  &  &  &  &  &  &  &  \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} & 0.5 & 1.13 & 0.5 & 1.10 & 0.4 & 1.04 & 0 ±0 & 1.09 ±0.04 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{AHA-WAM}
\label{part:aha_wam}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number &  &  &  &  &  &  &  &  \\
fold\_clothes &  &  &  &  &  &  &  &  \\
hang\_mugs &  &  &  &  &  &  &  &  \\
make\_toast &  &  &  &  &  &  &  &  \\
pack\_objects\_into\_box &  &  &  &  &  &  &  &  \\
pour\_liquid\_into\_cup &  &  &  &  &  &  &  &  \\
push\_T &  &  &  &  &  &  &  &  \\
sort\_nesting\_dolls\_by\_size &  &  &  &  &  &  &  &  \\
stack\_blocks &  &  &  &  &  &  &  &  \\
stack\_bowls &  &  &  &  &  &  &  &  \\
store\_laptop\_and\_headphones &  &  &  &  &  &  &  &  \\
sweep\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower &  &  &  &  &  &  &  &  \\
deposit\_coin &  &  &  &  &  &  &  &  \\
fasten\_screws &  &  &  &  &  &  &  &  \\
insert\_key &  &  &  &  &  &  &  &  \\
insert\_tubes &  &  &  &  &  &  &  &  \\
play\_Xylophone &  &  &  &  &  &  &  &  \\
plug\_in\_charger &  &  &  &  &  &  &  &  \\
pour\_balls\_into\_vase &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects &  &  &  &  &  &  &  &  \\
fill\_egg\_holder &  &  &  &  &  &  &  &  \\
fill\_pen\_holder &  &  &  &  &  &  &  &  \\
make\_kong &  &  &  &  &  &  &  &  \\
organize\_table &  &  &  &  &  &  &  &  \\
play\_stacking\_toy &  &  &  &  &  &  &  &  \\
play\_tic\_tac\_toe &  &  &  &  &  &  &  &  \\
put\_bottles\_into\_dustbin &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks &  &  &  &  &  &  &  &  \\
imitate\_sorting\_sequence &  &  &  &  &  &  &  &  \\
match\_and\_pick\_from\_conveyor &  &  &  &  &  &  &  &  \\
press\_by\_number &  &  &  &  &  &  &  &  \\
swap\_T &  &  &  &  &  &  &  &  \\
swap\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image &  &  &  &  &  &  &  &  \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{ABot-M0}
\label{part:abot_m0}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.60 & 0 & 0.70 & 0 & 1.70 & 0 ±0 & 1.00 ±0.55 \\
fold\_clothes & 6 & 7.20 & 10 & 14.80 & 18 & 24.40 & 11 ±6 & 15.47 ±8.60 \\
hang\_mugs & 0 & 3.80 & 0 & 2.60 & 0 & 2.30 & 0 ±0 & 2.90 ±0.75 \\
make\_toast & 0 & 4.00 & 0 & 2.00 & 0 & 2.00 & 0 ±0 & 2.67 ±1.00 \\
pack\_objects\_into\_box & 0 & 2.70 & 0 & 2.60 & 2 & 4.50 & 1 ±1 & 3.27 ±0.95 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 2 & 7.10 & 2 & 5.00 & 2 & 5.00 & 2 ±0 & 5.70 ±1.05 \\
stack\_bowls & 22 & 25.90 & 24 & 26.70 & 24 & 25.80 & 23 ±1 & 26.13 ±0.45 \\
store\_laptop\_and\_headphones & 2 & 11.60 & 0 & 6.40 & 0 & 4.80 & 1 ±1 & 7.60 ±3.40 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.00 & 0 & 0.40 & 0 & 0.20 & 0 ±0 & 0.20 ±0.20 \\
deposit\_coin & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
fasten\_screws & 0 & 2.60 & 0 & 3.20 & 0 & 3.20 & 0 ±0 & 3.00 ±0.30 \\
insert\_key & 0 & 11.70 & 0 & 13.80 & 0 & 14.10 & 0 ±0 & 13.20 ±1.20 \\
insert\_tubes & 2 & 18.00 & 0 & 10.00 & 0 & 8.40 & 1 ±1 & 12.13 ±4.80 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 2 & 2.00 & 1 ±1 & 0.67 ±1.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 2.10 & 0 & 2.40 & 0 & 1.40 & 0 ±0 & 1.97 ±0.50 \\
fill\_egg\_holder & 0 & 3.00 & 0 & 0.20 & 0 & 1.20 & 0 ±0 & 1.47 ±1.40 \\
fill\_pen\_holder & 0 & 0.20 & 0 & 0.50 & 0 & 1.20 & 0 ±0 & 0.63 ±0.50 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 5.00 & 0 & 6.00 & 0 & 3.50 & 0 ±0 & 4.83 ±1.25 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.80 & 0 & 3.40 & 0 & 3.00 & 0 ±0 & 2.40 ±1.30 \\
put\_bottles\_into\_dustbin & 8 & 25.20 & 4 & 24.70 & 6 & 25.30 & 6 ±2 & 25.07 ±0.30 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.30 & 0 & 0.50 & 0 & 2.10 & 0 ±0 & 0.97 ±0.90 \\
match\_and\_pick\_from\_conveyor & 10 & 10.00 & 12 & 12.00 & 8 & 8.00 & 10 ±2 & 10.00 ±2.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.20 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.33 ±0.10 \\
general\_pickup & 6 & 6.00 & 4 & 4.00 & 4 & 4.00 & 5 ±1 & 4.67 ±1.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 1.4 & 3.52 & 1.3 & 3.39 & 1.6 & 3.55 & 1 ±0 & 3.49 ±0.08 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Being-H0.5}
\label{part:being_h0_5}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number &  &  &  &  &  &  &  &  \\
fold\_clothes &  &  &  &  &  &  &  &  \\
hang\_mugs &  &  &  &  &  &  &  &  \\
make\_toast &  &  &  &  &  &  &  &  \\
pack\_objects\_into\_box &  &  &  &  &  &  &  &  \\
pour\_liquid\_into\_cup &  &  &  &  &  &  &  &  \\
push\_T &  &  &  &  &  &  &  &  \\
sort\_nesting\_dolls\_by\_size &  &  &  &  &  &  &  &  \\
stack\_blocks &  &  &  &  &  &  &  &  \\
stack\_bowls &  &  &  &  &  &  &  &  \\
store\_laptop\_and\_headphones &  &  &  &  &  &  &  &  \\
sweep\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower &  &  &  &  &  &  &  &  \\
deposit\_coin &  &  &  &  &  &  &  &  \\
fasten\_screws &  &  &  &  &  &  &  &  \\
insert\_key &  &  &  &  &  &  &  &  \\
insert\_tubes &  &  &  &  &  &  &  &  \\
play\_Xylophone &  &  &  &  &  &  &  &  \\
plug\_in\_charger &  &  &  &  &  &  &  &  \\
pour\_balls\_into\_vase &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects &  &  &  &  &  &  &  &  \\
fill\_egg\_holder &  &  &  &  &  &  &  &  \\
fill\_pen\_holder &  &  &  &  &  &  &  &  \\
make\_kong &  &  &  &  &  &  &  &  \\
organize\_table &  &  &  &  &  &  &  &  \\
play\_stacking\_toy &  &  &  &  &  &  &  &  \\
play\_tic\_tac\_toe &  &  &  &  &  &  &  &  \\
put\_bottles\_into\_dustbin &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks &  &  &  &  &  &  &  &  \\
imitate\_sorting\_sequence &  &  &  &  &  &  &  &  \\
match\_and\_pick\_from\_conveyor &  &  &  &  &  &  &  &  \\
press\_by\_number &  &  &  &  &  &  &  &  \\
swap\_T &  &  &  &  &  &  &  &  \\
swap\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image &  &  &  &  &  &  &  &  \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Dexbotic-DM0}
\label{part:dexbotic_dm0}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.10 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.03 ±0.05 \\
fold\_clothes & 0 & 0.40 & 0 & 8.40 & 0 & 0.00 & 0 ±0 & 2.93 ±4.20 \\
hang\_mugs & 0 & 1.20 & 0 & 0.90 & 0 & 0.00 & 0 ±0 & 0.70 ±0.60 \\
make\_toast & 0 & 0.00 & 0 & 1.00 & 0 & 0.00 & 0 ±0 & 0.33 ±0.50 \\
pack\_objects\_into\_box & 0 & 0.20 & 0 & 0.20 & 0 & 0.00 & 0 ±0 & 0.13 ±0.10 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_bowls & 0 & 0.60 & 0 & 1.80 & 0 & 0.00 & 0 ±0 & 0.80 ±0.90 \\
store\_laptop\_and\_headphones & 0 & 0.40 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.27 ±0.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
deposit\_coin & 0 & 0.00 & 0 & 0.80 & 0 & 0.40 & 0 ±0 & 0.40 ±0.40 \\
fasten\_screws & 0 & 0.80 & 0 & 1.00 & 0 & 0.00 & 0 ±0 & 0.60 ±0.50 \\
insert\_key & 0 & 3.30 & 0 & 1.50 & 0 & 3.30 & 0 ±0 & 2.70 ±0.90 \\
insert\_tubes & 0 & 1.20 & 0 & 2.40 & 0 & 0.00 & 0 ±0 & 1.20 ±1.20 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.00 & 0 & 0.60 & 0 & 0.00 & 0 ±0 & 0.20 ±0.30 \\
fill\_egg\_holder & 0 & 0.00 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 0.50 & 0 & 0.50 & 0 & 0.00 & 0 ±0 & 0.33 ±0.25 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.00 & 0 & 0.60 & 0 & 0.00 & 0 ±0 & 0.20 ±0.30 \\
put\_bottles\_into\_dustbin & 0 & 3.90 & 2 & 15.20 & 0 & 1.20 & 1 ±1 & 6.77 ±7.00 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.80 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.27 ±0.40 \\
imitate\_sorting\_sequence & 0 & 0.50 & 0 & 0.20 & 0 & 0.10 & 0 ±0 & 0.27 ±0.20 \\
match\_and\_pick\_from\_conveyor & 0 & 0.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.0 & 0.33 & 0.1 & 0.95 & 0.0 & 0.13 & 0 ±0 & 0.47 ±0.41 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Dexora-1B}
\label{part:dexora_1b}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number &  &  &  &  &  &  &  &  \\
fold\_clothes &  &  &  &  &  &  &  &  \\
hang\_mugs &  &  &  &  &  &  &  &  \\
make\_toast &  &  &  &  &  &  &  &  \\
pack\_objects\_into\_box &  &  &  &  &  &  &  &  \\
pour\_liquid\_into\_cup &  &  &  &  &  &  &  &  \\
push\_T &  &  &  &  &  &  &  &  \\
sort\_nesting\_dolls\_by\_size &  &  &  &  &  &  &  &  \\
stack\_blocks &  &  &  &  &  &  &  &  \\
stack\_bowls &  &  &  &  &  &  &  &  \\
store\_laptop\_and\_headphones &  &  &  &  &  &  &  &  \\
sweep\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower &  &  &  &  &  &  &  &  \\
deposit\_coin &  &  &  &  &  &  &  &  \\
fasten\_screws &  &  &  &  &  &  &  &  \\
insert\_key &  &  &  &  &  &  &  &  \\
insert\_tubes &  &  &  &  &  &  &  &  \\
play\_Xylophone &  &  &  &  &  &  &  &  \\
plug\_in\_charger &  &  &  &  &  &  &  &  \\
pour\_balls\_into\_vase &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects &  &  &  &  &  &  &  &  \\
fill\_egg\_holder &  &  &  &  &  &  &  &  \\
fill\_pen\_holder &  &  &  &  &  &  &  &  \\
make\_kong &  &  &  &  &  &  &  &  \\
organize\_table &  &  &  &  &  &  &  &  \\
play\_stacking\_toy &  &  &  &  &  &  &  &  \\
play\_tic\_tac\_toe &  &  &  &  &  &  &  &  \\
put\_bottles\_into\_dustbin &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks &  &  &  &  &  &  &  &  \\
imitate\_sorting\_sequence &  &  &  &  &  &  &  &  \\
match\_and\_pick\_from\_conveyor &  &  &  &  &  &  &  &  \\
press\_by\_number &  &  &  &  &  &  &  &  \\
swap\_T &  &  &  &  &  &  &  &  \\
swap\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image &  &  &  &  &  &  &  &  \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{EventVLA}
\label{part:eventvla}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 1.60 & 0 & 1.10 & 0 & 1.60 & 0 ±0 & 1.43 ±0.25 \\
fold\_clothes & 8 & 8.80 & 14 & 16.80 & 10 & 13.60 & 11 ±3 & 13.07 ±4.00 \\
hang\_mugs & 0 & 2.10 & 0 & 1.20 & 0 & 1.80 & 0 ±0 & 1.70 ±0.45 \\
make\_toast & 0 & 0.50 & 0 & 0.50 & 0 & 1.00 & 0 ±0 & 0.67 ±0.25 \\
pack\_objects\_into\_box & 0 & 2.20 & 0 & 0.20 & 0 & 1.80 & 0 ±0 & 1.40 ±1.00 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 3.90 & 4 & 8.20 & 2 & 7.10 & 2 ±2 & 6.40 ±2.15 \\
stack\_bowls & 10 & 13.00 & 6 & 10.20 & 4 & 8.20 & 7 ±3 & 10.47 ±2.40 \\
store\_laptop\_and\_headphones & 2 & 10.40 & 4 & 14.80 & 6 & 11.20 & 4 ±2 & 12.13 ±2.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
deposit\_coin & 0 & 2.80 & 0 & 2.00 & 0 & 2.00 & 0 ±0 & 2.27 ±0.40 \\
fasten\_screws & 0 & 5.80 & 0 & 3.00 & 0 & 1.60 & 0 ±0 & 3.47 ±2.10 \\
insert\_key & 0 & 12.60 & 0 & 12.60 & 0 & 14.40 & 0 ±0 & 13.20 ±0.90 \\
insert\_tubes & 28 & 48.00 & 44 & 56.40 & 46 & 62.00 & 39 ±9 & 55.47 ±7.00 \\
play\_Xylophone & 2 & 2.00 & 18 & 18.00 & 0 & 0.00 & 7 ±9 & 6.67 ±9.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 1.20 & 0 & 0.60 & 0 & 0.00 & 0 ±0 & 0.60 ±0.60 \\
fill\_egg\_holder & 0 & 0.60 & 0 & 1.50 & 0 & 1.50 & 0 ±0 & 1.20 ±0.45 \\
fill\_pen\_holder & 0 & 0.20 & 0 & 1.10 & 0 & 0.60 & 0 ±0 & 0.63 ±0.45 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 2.50 & 0 & 4.00 & 0 & 3.50 & 0 ±0 & 3.33 ±0.75 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.20 & 0 ±0 & 0.07 ±0.10 \\
play\_tic\_tac\_toe & 4 & 24.40 & 4 & 23.80 & 4 & 21.20 & 4 ±0 & 23.13 ±1.60 \\
put\_bottles\_into\_dustbin & 2 & 12.60 & 2 & 9.80 & 4 & 11.90 & 3 ±1 & 11.43 ±1.40 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 1.00 & 0 & 0.90 & 0 & 0.70 & 0 ±0 & 0.87 ±0.15 \\
match\_and\_pick\_from\_conveyor & 6 & 6.00 & 18 & 18.00 & 10 & 10.00 & 11 ±6 & 11.33 ±6.00 \\
press\_by\_number & 2 & 2.00 & 2 & 2.00 & 4 & 4.00 & 3 ±1 & 2.67 ±1.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 14 & 14.00 & 12 & 12.00 & 18 & 18.00 & 15 ±3 & 14.67 ±3.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 2 & 2.00 & 8 & 8.00 & 6 & 6.00 & 5 ±3 & 5.33 ±3.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 2 & 2.40 & 0 & 0.40 & 0 & 0.40 & 1 ±1 & 1.07 ±1.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 2.0 & 4.35 & 3.2 & 5.41 & 2.7 & 4.86 & 3 ±1 & 4.87 ±0.53 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{FastWAM}
\label{part:fastwam}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.30 & 0 & 0.50 & 0 & 0.80 & 0 ±0 & 0.53 ±0.25 \\
fold\_clothes & 22 & 25.60 & 8 & 13.60 & 6 & 12.00 & 12 ±8 & 17.07 ±6.80 \\
hang\_mugs & 0 & 1.20 & 0 & 1.50 & 0 & 0.60 & 0 ±0 & 1.10 ±0.45 \\
make\_toast & 0 & 0.00 & 0 & 4.00 & 0 & 0.00 & 0 ±0 & 1.33 ±2.00 \\
pack\_objects\_into\_box & 0 & 1.70 & 0 & 0.80 & 0 & 2.20 & 0 ±0 & 1.57 ±0.70 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 2.10 & 0 & 3.60 & 0 & 2.40 & 0 ±0 & 2.70 ±0.75 \\
stack\_bowls & 2 & 3.50 & 0 & 2.40 & 2 & 4.10 & 1 ±1 & 3.33 ±0.85 \\
store\_laptop\_and\_headphones & 0 & 0.40 & 0 & 0.00 & 0 & 0.80 & 0 ±0 & 0.40 ±0.40 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 2.80 & 0 & 3.80 & 0 & 6.80 & 0 ±0 & 4.47 ±2.00 \\
deposit\_coin & 0 & 2.00 & 0 & 2.40 & 0 & 4.00 & 0 ±0 & 2.80 ±1.00 \\
fasten\_screws & 0 & 0.40 & 0 & 0.80 & 0 & 0.00 & 0 ±0 & 0.40 ±0.40 \\
insert\_key & 0 & 3.90 & 0 & 4.50 & 0 & 4.50 & 0 ±0 & 4.30 ±0.30 \\
insert\_tubes & 0 & 4.00 & 0 & 3.60 & 0 & 3.60 & 0 ±0 & 3.73 ±0.20 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 4 & 4.60 & 0 & 1.80 & 0 & 2.90 & 1 ±2 & 3.10 ±1.40 \\
fill\_egg\_holder & 0 & 0.80 & 0 & 0.60 & 0 & 0.80 & 0 ±0 & 0.73 ±0.10 \\
fill\_pen\_holder & 0 & 2.50 & 0 & 4.40 & 0 & 5.30 & 0 ±0 & 4.07 ±1.40 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 7.50 & 0 & 9.00 & 0 & 7.00 & 0 ±0 & 7.83 ±1.00 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
put\_bottles\_into\_dustbin & 34 & 51.20 & 52 & 66.20 & 34 & 54.70 & 40 ±9 & 57.37 ±7.50 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.50 & 0 & 0.60 & 0 & 0.80 & 0 ±0 & 0.63 ±0.15 \\
match\_and\_pick\_from\_conveyor & 10 & 10.00 & 34 & 34.00 & 18 & 18.00 & 21 ±12 & 20.67 ±12.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 0 & 0.00 & 4 & 4.00 & 6 & 6.00 & 3 ±3 & 3.33 ±3.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 1.7 & 2.98 & 2.3 & 3.86 & 1.6 & 3.27 & 2 ±0 & 3.37 ±0.44 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{GO1}
\label{part:go1}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fold\_clothes & 4 & 6.40 & 6 & 7.60 & 6 & 7.60 & 5 ±1 & 7.20 ±0.60 \\
hang\_mugs & 0 & 0.60 & 0 & 0.30 & 0 & 0.60 & 0 ±0 & 0.50 ±0.15 \\
make\_toast & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pack\_objects\_into\_box & 0 & 0.20 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.20 ±0.20 \\
pour\_liquid\_into\_cup & 2 & 2.00 & 6 & 6.00 & 6 & 6.00 & 5 ±2 & 4.67 ±2.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.30 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.10 ±0.15 \\
stack\_bowls & 4 & 4.60 & 6 & 7.50 & 4 & 4.90 & 5 ±1 & 5.67 ±1.45 \\
store\_laptop\_and\_headphones & 0 & 0.80 & 0 & 0.80 & 0 & 0.40 & 0 ±0 & 0.67 ±0.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 6.00 & 6 & 10.40 & 4 & 10.20 & 3 ±3 & 8.87 ±2.20 \\
deposit\_coin & 0 & 0.40 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.40 ±0.00 \\
fasten\_screws & 0 & 1.20 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.53 ±0.60 \\
insert\_key & 0 & 0.60 & 0 & 2.40 & 0 & 1.20 & 0 ±0 & 1.40 ±0.90 \\
insert\_tubes & 0 & 0.80 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.40 ±0.40 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.00 & 0 & 0.00 & 0 & 0.30 & 0 ±0 & 0.10 ±0.15 \\
fill\_egg\_holder & 0 & 0.40 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.27 ±0.20 \\
fill\_pen\_holder & 0 & 0.70 & 0 & 1.30 & 0 & 0.40 & 0 ±0 & 0.80 ±0.45 \\
make\_kong & 2 & 2.00 & 4 & 4.00 & 0 & 0.00 & 2 ±2 & 2.00 ±2.00 \\
organize\_table & 0 & 0.00 & 0 & 1.00 & 0 & 0.00 & 0 ±0 & 0.33 ±0.50 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.80 & 0 & 1.60 & 0 & 1.80 & 0 ±0 & 1.40 ±0.50 \\
put\_bottles\_into\_dustbin & 0 & 3.10 & 0 & 5.30 & 0 & 4.00 & 0 ±0 & 4.13 ±1.10 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.10 & 0 & 0.00 & 0 ±0 & 0.03 ±0.05 \\
imitate\_sorting\_sequence & 0 & 0.20 & 0 & 0.10 & 0 & 0.20 & 0 ±0 & 0.17 ±0.05 \\
match\_and\_pick\_from\_conveyor & 0 & 0.00 & 6 & 6.00 & 6 & 6.00 & 4 ±3 & 4.00 ±3.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 2 & 2.00 & 0 & 0.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.3 & 0.79 & 0.8 & 1.34 & 0.6 & 1.05 & 1 ±0 & 1.06 ±0.28 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{GR00T-N1.7}
\label{part:gr00t_n17}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.10 & 0 & 0.00 & 0 & 0.10 & 0 ±0 & 0.07 ±0.05 \\
fold\_clothes & 0 & 1.20 & 0 & 1.20 & 4 & 5.20 & 1 ±2 & 2.53 ±2.00 \\
hang\_mugs & 0 & 0.60 & 0 & 1.80 & 0 & 1.20 & 0 ±0 & 1.20 ±0.60 \\
make\_toast & 0 & 2.00 & 0 & 1.00 & 0 & 0.50 & 0 ±0 & 1.17 ±0.75 \\
pack\_objects\_into\_box & 0 & 1.10 & 0 & 0.80 & 0 & 0.70 & 0 ±0 & 0.87 ±0.20 \\
pour\_liquid\_into\_cup & 2 & 2.00 & 8 & 8.00 & 4 & 4.00 & 5 ±3 & 4.67 ±3.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.30 & 0 & 0.00 & 0 ±0 & 0.10 ±0.15 \\
stack\_bowls & 12 & 14.40 & 6 & 8.70 & 8 & 11.30 & 9 ±3 & 11.47 ±2.85 \\
store\_laptop\_and\_headphones & 0 & 6.00 & 0 & 2.00 & 0 & 3.60 & 0 ±0 & 3.87 ±2.00 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 1.20 & 0 & 0.60 & 0 & 0.40 & 0 ±0 & 0.73 ±0.40 \\
deposit\_coin & 2 & 4.00 & 2 & 4.00 & 0 & 1.60 & 1 ±1 & 3.20 ±1.20 \\
fasten\_screws & 0 & 0.40 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.40 ±0.00 \\
insert\_key & 0 & 8.10 & 0 & 8.40 & 0 & 9.00 & 0 ±0 & 8.50 ±0.45 \\
insert\_tubes & 0 & 3.60 & 0 & 3.20 & 0 & 3.60 & 0 ±0 & 3.47 ±0.20 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 6 & 6.00 & 6 & 6.00 & 4 ±3 & 4.00 ±3.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 2.70 & 0 & 2.70 & 0 & 2.90 & 0 ±0 & 2.77 ±0.10 \\
fill\_egg\_holder & 0 & 1.00 & 0 & 1.40 & 0 & 1.10 & 0 ±0 & 1.17 ±0.20 \\
fill\_pen\_holder & 0 & 4.00 & 4 & 11.00 & 0 & 7.20 & 1 ±2 & 7.40 ±3.50 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 9.00 & 0 & 7.00 & 0 & 9.50 & 0 ±0 & 8.50 ±1.25 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.60 & 0 & 3.00 & 0 & 1.20 & 0 ±0 & 1.60 ±1.20 \\
put\_bottles\_into\_dustbin & 28 & 44.90 & 38 & 54.20 & 16 & 35.80 & 27 ±11 & 44.97 ±9.20 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.90 & 0 & 1.00 & 0 & 1.00 & 0 ±0 & 0.97 ±0.05 \\
imitate\_sorting\_sequence & 0 & 0.00 & 0 & 0.10 & 0 & 0.00 & 0 ±0 & 0.03 ±0.05 \\
match\_and\_pick\_from\_conveyor & 6 & 6.00 & 4 & 4.00 & 6 & 6.00 & 5 ±1 & 5.33 ±1.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.20 & 0 & 0.00 & 0 & 0.20 & 0 ±0 & 0.13 ±0.10 \\
general\_pickup & 0 & 0.00 & 2 & 2.00 & 2 & 2.00 & 1 ±1 & 1.33 ±1.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 1.2 & 2.71 & 1.7 & 3.16 & 1.1 & 2.73 & 1 ±0 & 2.87 ±0.22 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{GalaxeaVLA}
\label{part:galaxeavla}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.30 & 0 & 0.10 & 0 & 0.10 & 0 ±0 & 0.17 ±0.10 \\
fold\_clothes & 8 & 10.00 & 12 & 13.60 & 6 & 8.00 & 9 ±3 & 10.53 ±2.80 \\
hang\_mugs & 0 & 3.90 & 0 & 3.60 & 0 & 3.70 & 0 ±0 & 3.73 ±0.15 \\
make\_toast & 0 & 2.50 & 0 & 3.00 & 0 & 3.00 & 0 ±0 & 2.83 ±0.25 \\
pack\_objects\_into\_box & 0 & 1.70 & 0 & 2.20 & 0 & 3.20 & 0 ±0 & 2.37 ±0.75 \\
pour\_liquid\_into\_cup & 6 & 6.00 & 2 & 2.00 & 10 & 10.00 & 6 ±4 & 6.00 ±4.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 2 & 2.00 & 2 & 2.00 & 2 & 2.00 & 2 ±0 & 2.00 ±0.00 \\
stack\_blocks & 0 & 1.20 & 0 & 0.60 & 0 & 1.20 & 0 ±0 & 1.00 ±0.30 \\
stack\_bowls & 24 & 25.50 & 12 & 15.90 & 14 & 17.90 & 17 ±6 & 19.77 ±4.80 \\
store\_laptop\_and\_headphones & 2 & 4.40 & 0 & 9.20 & 0 & 4.40 & 1 ±1 & 6.00 ±2.40 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 12 & 18.40 & 6 & 14.60 & 6 & 19.40 & 8 ±3 & 17.47 ±2.40 \\
deposit\_coin & 0 & 1.60 & 0 & 1.20 & 0 & 1.20 & 0 ±0 & 1.33 ±0.20 \\
fasten\_screws & 0 & 0.80 & 0 & 1.20 & 0 & 0.80 & 0 ±0 & 0.93 ±0.20 \\
insert\_key & 0 & 8.70 & 0 & 10.80 & 0 & 9.30 & 0 ±0 & 9.60 ±1.05 \\
insert\_tubes & 8 & 20.40 & 4 & 18.40 & 14 & 25.60 & 9 ±5 & 21.47 ±3.60 \\
play\_Xylophone & 8 & 8.00 & 2 & 2.00 & 6 & 6.00 & 5 ±3 & 5.33 ±3.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 8 & 8.00 & 8 & 8.00 & 10 & 10.00 & 9 ±1 & 8.67 ±1.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 2 & 5.00 & 0 & 3.00 & 2 & 4.80 & 1 ±1 & 4.27 ±1.00 \\
fill\_egg\_holder & 0 & 1.90 & 0 & 1.00 & 0 & 3.10 & 0 ±0 & 2.00 ±1.05 \\
fill\_pen\_holder & 2 & 12.90 & 0 & 11.90 & 2 & 12.20 & 1 ±1 & 12.33 ±0.50 \\
make\_kong & 4 & 4.00 & 12 & 12.00 & 10 & 10.00 & 9 ±4 & 8.67 ±4.00 \\
organize\_table & 0 & 24.00 & 0 & 17.00 & 0 & 22.00 & 0 ±0 & 21.00 ±3.50 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 3.20 & 0 & 2.40 & 0 & 4.00 & 0 ±0 & 3.20 ±0.80 \\
put\_bottles\_into\_dustbin & 36 & 52.00 & 36 & 51.80 & 28 & 44.30 & 33 ±4 & 49.37 ±3.85 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 6 & 12.90 & 4 & 11.70 & 0 & 8.10 & 3 ±3 & 10.90 ±2.40 \\
imitate\_sorting\_sequence & 0 & 0.20 & 0 & 0.10 & 0 & 0.00 & 0 ±0 & 0.10 ±0.10 \\
match\_and\_pick\_from\_conveyor & 10 & 10.00 & 6 & 6.00 & 8 & 8.00 & 8 ±2 & 8.00 ±2.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.20 & 0 ±0 & 0.07 ±0.10 \\
general\_pickup & 4 & 4.00 & 10 & 10.00 & 2 & 2.00 & 5 ±4 & 5.33 ±4.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.50 & 0 & 0.00 & 0 ±0 & 0.17 ±0.25 \\
\hline
\textbf{Avg} & 3.4 & 6.04 & 2.8 & 5.61 & 2.9 & 5.82 & 3 ±0 & 5.82 ±0.21 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{GigaWorldPolicy}
\label{part:gigaworldpolicy}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.10 & 0 & 0.10 & 0 & 0.10 & 0 ±0 & 0.10 ±0.00 \\
fold\_clothes & 4 & 8.00 & 12 & 14.80 & 6 & 13.20 & 7 ±4 & 12.00 ±3.40 \\
hang\_mugs & 0 & 3.80 & 0 & 4.90 & 0 & 4.70 & 0 ±0 & 4.47 ±0.55 \\
make\_toast & 0 & 4.50 & 0 & 1.00 & 2 & 4.00 & 1 ±1 & 3.17 ±1.75 \\
pack\_objects\_into\_box & 0 & 2.90 & 0 & 6.20 & 2 & 5.60 & 1 ±1 & 4.90 ±1.65 \\
pour\_liquid\_into\_cup & 2 & 2.00 & 8 & 8.00 & 8 & 8.00 & 6 ±3 & 6.00 ±3.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 2 & 2.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 1.33 ±1.00 \\
stack\_blocks & 0 & 3.30 & 0 & 1.80 & 0 & 2.70 & 0 ±0 & 2.60 ±0.75 \\
stack\_bowls & 16 & 19.00 & 22 & 25.30 & 12 & 15.90 & 17 ±5 & 20.07 ±4.70 \\
store\_laptop\_and\_headphones & 2 & 10.40 & 4 & 10.00 & 0 & 8.00 & 2 ±2 & 9.47 ±1.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 6 & 20.40 & 4 & 13.00 & 10 & 22.40 & 7 ±3 & 18.60 ±4.70 \\
deposit\_coin & 0 & 3.20 & 0 & 3.20 & 0 & 3.60 & 0 ±0 & 3.33 ±0.20 \\
fasten\_screws & 0 & 3.40 & 0 & 1.60 & 0 & 3.00 & 0 ±0 & 2.67 ±0.90 \\
insert\_key & 0 & 10.80 & 0 & 10.80 & 0 & 11.40 & 0 ±0 & 11.00 ±0.30 \\
insert\_tubes & 0 & 5.20 & 0 & 3.20 & 2 & 10.40 & 1 ±1 & 6.27 ±3.60 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 2 & 2.00 & 1 ±1 & 0.67 ±1.00 \\
pour\_balls\_into\_vase & 8 & 8.00 & 8 & 8.00 & 4 & 4.00 & 7 ±2 & 6.67 ±2.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 2 & 5.00 & 0 & 3.80 & 6 & 9.60 & 3 ±3 & 6.13 ±2.90 \\
fill\_egg\_holder & 0 & 1.70 & 0 & 1.30 & 0 & 1.30 & 0 ±0 & 1.43 ±0.20 \\
fill\_pen\_holder & 0 & 11.10 & 2 & 14.70 & 0 & 12.70 & 1 ±1 & 12.83 ±1.80 \\
make\_kong & 0 & 0.00 & 6 & 6.00 & 0 & 0.00 & 2 ±3 & 2.00 ±3.00 \\
organize\_table & 2 & 24.00 & 0 & 27.00 & 2 & 24.00 & 1 ±1 & 25.00 ±1.50 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 1.20 & 0 & 1.00 & 0 & 1.20 & 0 ±0 & 1.13 ±0.10 \\
put\_bottles\_into\_dustbin & 64 & 74.40 & 70 & 79.30 & 60 & 73.00 & 65 ±5 & 75.57 ±3.15 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 6.00 & 0 & 5.70 & 0 & 6.40 & 0 ±0 & 6.03 ±0.35 \\
imitate\_sorting\_sequence & 0 & 0.90 & 0 & 0.80 & 0 & 2.40 & 0 ±0 & 1.37 ±0.80 \\
match\_and\_pick\_from\_conveyor & 10 & 10.00 & 18 & 18.00 & 12 & 12.00 & 13 ±4 & 13.33 ±4.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.20 & 0 & 0.60 & 0 & 0.20 & 0 ±0 & 0.33 ±0.20 \\
general\_pickup & 4 & 4.00 & 2 & 2.00 & 6 & 6.00 & 4 ±2 & 4.00 ±2.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 2.9 & 5.85 & 3.8 & 6.53 & 3.2 & 6.38 & 3 ±0 & 6.25 ±0.34 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{H\_RDT}
\label{part:h_rdt}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number &  &  &  &  &  &  &  &  \\
fold\_clothes &  &  &  &  &  &  &  &  \\
hang\_mugs &  &  &  &  &  &  &  &  \\
make\_toast &  &  &  &  &  &  &  &  \\
pack\_objects\_into\_box &  &  &  &  &  &  &  &  \\
pour\_liquid\_into\_cup &  &  &  &  &  &  &  &  \\
push\_T &  &  &  &  &  &  &  &  \\
sort\_nesting\_dolls\_by\_size &  &  &  &  &  &  &  &  \\
stack\_blocks &  &  &  &  &  &  &  &  \\
stack\_bowls &  &  &  &  &  &  &  &  \\
store\_laptop\_and\_headphones &  &  &  &  &  &  &  &  \\
sweep\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower &  &  &  &  &  &  &  &  \\
deposit\_coin &  &  &  &  &  &  &  &  \\
fasten\_screws &  &  &  &  &  &  &  &  \\
insert\_key &  &  &  &  &  &  &  &  \\
insert\_tubes &  &  &  &  &  &  &  &  \\
play\_Xylophone &  &  &  &  &  &  &  &  \\
plug\_in\_charger &  &  &  &  &  &  &  &  \\
pour\_balls\_into\_vase &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects &  &  &  &  &  &  &  &  \\
fill\_egg\_holder &  &  &  &  &  &  &  &  \\
fill\_pen\_holder &  &  &  &  &  &  &  &  \\
make\_kong &  &  &  &  &  &  &  &  \\
organize\_table &  &  &  &  &  &  &  &  \\
play\_stacking\_toy &  &  &  &  &  &  &  &  \\
play\_tic\_tac\_toe &  &  &  &  &  &  &  &  \\
put\_bottles\_into\_dustbin &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks &  &  &  &  &  &  &  &  \\
imitate\_sorting\_sequence &  &  &  &  &  &  &  &  \\
match\_and\_pick\_from\_conveyor &  &  &  &  &  &  &  &  \\
press\_by\_number &  &  &  &  &  &  &  &  \\
swap\_T &  &  &  &  &  &  &  &  \\
swap\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image &  &  &  &  &  &  &  &  \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{InternVLA-A1}
\label{part:internvla_a1}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.50 & 0 & 0.30 & 0 & 0.00 & 0 ±0 & 0.27 ±0.25 \\
fold\_clothes & 8 & 10.40 & 10 & 14.00 & 4 & 8.00 & 7 ±3 & 10.80 ±3.00 \\
hang\_mugs & 0 & 1.20 & 0 & 1.50 & 0 & 0.90 & 0 ±0 & 1.20 ±0.30 \\
make\_toast & 0 & 0.00 & 0 & 1.00 & 0 & 0.50 & 0 ±0 & 0.50 ±0.50 \\
pack\_objects\_into\_box & 0 & 1.10 & 0 & 0.20 & 0 & 1.30 & 0 ±0 & 0.87 ±0.55 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 4 & 4.00 & 1 ±2 & 1.33 ±2.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 1.20 & 0 & 1.50 & 0 & 1.80 & 0 ±0 & 1.50 ±0.30 \\
stack\_bowls & 16 & 18.40 & 12 & 15.60 & 12 & 16.20 & 13 ±2 & 16.73 ±1.40 \\
store\_laptop\_and\_headphones & 0 & 0.80 & 0 & 0.40 & 0 & 2.40 & 0 ±0 & 1.20 ±1.00 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 6 & 11.40 & 2 & 7.00 & 2 & 7.20 & 3 ±2 & 8.53 ±2.20 \\
deposit\_coin & 0 & 0.00 & 0 & 0.00 & 0 & 2.00 & 0 ±0 & 0.67 ±1.00 \\
fasten\_screws & 0 & 0.00 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
insert\_key & 0 & 6.30 & 0 & 3.60 & 0 & 6.60 & 0 ±0 & 5.50 ±1.50 \\
insert\_tubes & 0 & 6.40 & 0 & 7.20 & 0 & 2.00 & 0 ±0 & 5.20 ±2.60 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 4 & 4.00 & 2 & 2.00 & 6 & 6.00 & 4 ±2 & 4.00 ±2.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.60 & 0 & 0.90 & 0 & 0.90 & 0 ±0 & 0.80 ±0.15 \\
fill\_egg\_holder & 0 & 0.20 & 0 & 0.80 & 0 & 1.20 & 0 ±0 & 0.73 ±0.50 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 1.20 & 0 ±0 & 0.40 ±0.60 \\
make\_kong & 0 & 0.00 & 2 & 2.00 & 4 & 4.00 & 2 ±2 & 2.00 ±2.00 \\
organize\_table & 0 & 5.50 & 0 & 1.50 & 0 & 3.50 & 0 ±0 & 3.50 ±2.00 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.60 & 0 & 1.40 & 0 & 1.00 & 0 ±0 & 1.00 ±0.40 \\
put\_bottles\_into\_dustbin & 10 & 33.00 & 6 & 31.20 & 6 & 25.40 & 7 ±2 & 29.87 ±3.80 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.20 & 0 & 0.60 & 2 & 5.00 & 1 ±1 & 1.93 ±2.40 \\
imitate\_sorting\_sequence & 0 & 0.10 & 0 & 0.10 & 0 & 0.40 & 0 ±0 & 0.20 ±0.15 \\
match\_and\_pick\_from\_conveyor & 8 & 8.00 & 4 & 4.00 & 10 & 10.00 & 7 ±3 & 7.33 ±3.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 0 & 0.00 & 2 & 2.00 & 2 & 2.00 & 1 ±1 & 1.33 ±1.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 1.2 & 2.62 & 1.0 & 2.36 & 1.2 & 2.70 & 1 ±0 & 2.56 ±0.17 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{LDA-1B}
\label{part:lda_1b}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.10 & 0 & 0.10 & 0 & 0.20 & 0 ±0 & 0.13 ±0.05 \\
fold\_clothes & 6 & 8.80 & 0 & 2.40 & 8 & 10.80 & 5 ±4 & 7.33 ±4.20 \\
hang\_mugs & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_toast & 0 & 1.00 & 0 & 0.50 & 0 & 0.00 & 0 ±0 & 0.50 ±0.50 \\
pack\_objects\_into\_box & 0 & 0.40 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.30 & 0 & 0.30 & 0 & 0.00 & 0 ±0 & 0.20 ±0.15 \\
stack\_bowls & 0 & 1.20 & 0 & 1.50 & 0 & 0.00 & 0 ±0 & 0.90 ±0.75 \\
store\_laptop\_and\_headphones & 0 & 0.40 & 0 & 1.20 & 0 & 0.00 & 0 ±0 & 0.53 ±0.60 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 2.80 & 0 & 2.20 & 0 & 3.80 & 0 ±0 & 2.93 ±0.80 \\
deposit\_coin & 0 & 2.40 & 0 & 1.60 & 0 & 1.60 & 0 ±0 & 1.87 ±0.40 \\
fasten\_screws & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_key & 0 & 6.60 & 0 & 6.00 & 0 & 0.00 & 0 ±0 & 4.20 ±3.30 \\
insert\_tubes & 0 & 0.00 & 0 & 4.00 & 0 & 0.00 & 0 ±0 & 1.33 ±2.00 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_egg\_holder & 0 & 0.20 & 0 & 0.20 & 0 & 0.40 & 0 ±0 & 0.27 ±0.10 \\
fill\_pen\_holder & 0 & 0.20 & 0 & 0.70 & 0 & 0.40 & 0 ±0 & 0.43 ±0.25 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 0.50 & 0 & 2.00 & 0 & 0.00 & 0 ±0 & 0.83 ±1.00 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.80 & 0 & 0.60 & 0 & 0.00 & 0 ±0 & 0.47 ±0.40 \\
put\_bottles\_into\_dustbin & 2 & 6.50 & 0 & 7.10 & 0 & 0.40 & 1 ±1 & 4.67 ±3.35 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 3.50 & 0 & 3.90 & 0 & 2.40 & 0 ±0 & 3.27 ±0.75 \\
imitate\_sorting\_sequence & 0 & 0.20 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.07 ±0.10 \\
match\_and\_pick\_from\_conveyor & 2 & 2.00 & 4 & 4.00 & 2 & 2.00 & 3 ±1 & 2.67 ±1.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 2 & 2.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 1.33 ±1.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.3 & 0.95 & 0.1 & 0.96 & 0.2 & 0.52 & 0 ±0 & 0.81 ±0.22 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{MolmoACT2}
\label{part:molmoact2}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.10 & 0 ±0 & 0.03 ±0.05 \\
fold\_clothes & 0 & 2.40 & 2 & 5.20 & 0 & 2.80 & 1 ±1 & 3.47 ±1.40 \\
hang\_mugs & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_toast & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pack\_objects\_into\_box & 0 & 0.40 & 0 & 0.40 & 0 & 0.20 & 0 ±0 & 0.33 ±0.10 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.60 & 0 & 0.60 & 0 ±0 & 0.40 ±0.30 \\
stack\_bowls & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_laptop\_and\_headphones & 0 & 0.80 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.40 ±0.40 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
deposit\_coin & 0 & 0.40 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.27 ±0.20 \\
fasten\_screws & 0 & 0.00 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.27 ±0.20 \\
insert\_key & 0 & 4.50 & 0 & 1.20 & 0 & 3.60 & 0 ±0 & 3.10 ±1.65 \\
insert\_tubes & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 1.80 & 0 & 1.50 & 0 & 0.90 & 0 ±0 & 1.40 ±0.45 \\
fill\_egg\_holder & 0 & 1.40 & 0 & 1.40 & 0 & 0.40 & 0 ±0 & 1.07 ±0.50 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 12.50 & 0 & 11.50 & 0 & 10.00 & 0 ±0 & 11.33 ±1.25 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 1.00 & 0 & 0.80 & 0 & 0.20 & 0 ±0 & 0.67 ±0.40 \\
put\_bottles\_into\_dustbin & 0 & 4.60 & 0 & 2.10 & 0 & 5.50 & 0 ±0 & 4.07 ±1.70 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.30 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.10 ±0.15 \\
match\_and\_pick\_from\_conveyor & 8 & 8.00 & 4 & 4.00 & 6 & 6.00 & 6 ±2 & 6.00 ±2.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.60 & 0 & 0.80 & 0 & 0.40 & 0 ±0 & 0.60 ±0.20 \\
general\_pickup & 8 & 8.00 & 4 & 4.00 & 8 & 8.00 & 7 ±2 & 6.67 ±2.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.4 & 1.11 & 0.2 & 0.81 & 0.3 & 0.95 & 0 ±0 & 0.96 ±0.15 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Motus}
\label{part:motus}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number &  &  &  &  &  &  &  &  \\
fold\_clothes &  &  &  &  &  &  &  &  \\
hang\_mugs &  &  &  &  &  &  &  &  \\
make\_toast &  &  &  &  &  &  &  &  \\
pack\_objects\_into\_box &  &  &  &  &  &  &  &  \\
pour\_liquid\_into\_cup &  &  &  &  &  &  &  &  \\
push\_T &  &  &  &  &  &  &  &  \\
sort\_nesting\_dolls\_by\_size &  &  &  &  &  &  &  &  \\
stack\_blocks &  &  &  &  &  &  &  &  \\
stack\_bowls &  &  &  &  &  &  &  &  \\
store\_laptop\_and\_headphones &  &  &  &  &  &  &  &  \\
sweep\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower &  &  &  &  &  &  &  &  \\
deposit\_coin &  &  &  &  &  &  &  &  \\
fasten\_screws &  &  &  &  &  &  &  &  \\
insert\_key &  &  &  &  &  &  &  &  \\
insert\_tubes &  &  &  &  &  &  &  &  \\
play\_Xylophone &  &  &  &  &  &  &  &  \\
plug\_in\_charger &  &  &  &  &  &  &  &  \\
pour\_balls\_into\_vase &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects &  &  &  &  &  &  &  &  \\
fill\_egg\_holder &  &  &  &  &  &  &  &  \\
fill\_pen\_holder &  &  &  &  &  &  &  &  \\
make\_kong &  &  &  &  &  &  &  &  \\
organize\_table &  &  &  &  &  &  &  &  \\
play\_stacking\_toy &  &  &  &  &  &  &  &  \\
play\_tic\_tac\_toe &  &  &  &  &  &  &  &  \\
put\_bottles\_into\_dustbin &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks &  &  &  &  &  &  &  &  \\
imitate\_sorting\_sequence &  &  &  &  &  &  &  &  \\
match\_and\_pick\_from\_conveyor &  &  &  &  &  &  &  &  \\
press\_by\_number &  &  &  &  &  &  &  &  \\
swap\_T &  &  &  &  &  &  &  &  \\
swap\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image &  &  &  &  &  &  &  &  \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{OpenVLA-OFT}
\label{part:openvla_oft}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fold\_clothes & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
hang\_mugs & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_toast & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pack\_objects\_into\_box & 0 & 0.20 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.07 ±0.10 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_bowls & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_laptop\_and\_headphones & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
deposit\_coin & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fasten\_screws & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_key & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_tubes & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_egg\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
put\_bottles\_into\_dustbin & 0 & 0.40 & 0 & 0.20 & 0 & 0.00 & 0 ±0 & 0.20 ±0.20 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
match\_and\_pick\_from\_conveyor & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.0 & 0.01 & 0.0 & 0.00 & 0.0 & 0.00 & 0 ±0 & 0.01 ±0.01 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Pi-0}
\label{part:pi_0}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.40 & 0 & 0.10 & 0 & 0.30 & 0 ±0 & 0.27 ±0.15 \\
fold\_clothes & 0 & 2.80 & 8 & 15.20 & 12 & 18.80 & 7 ±6 & 12.27 ±8.00 \\
hang\_mugs & 0 & 1.20 & 0 & 3.20 & 0 & 2.30 & 0 ±0 & 2.23 ±1.00 \\
make\_toast & 0 & 1.00 & 0 & 0.00 & 0 & 0.50 & 0 ±0 & 0.50 ±0.50 \\
pack\_objects\_into\_box & 0 & 0.20 & 0 & 1.60 & 0 & 1.40 & 0 ±0 & 1.07 ±0.70 \\
pour\_liquid\_into\_cup & 4 & 4.00 & 12 & 12.00 & 8 & 8.00 & 8 ±4 & 8.00 ±4.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.90 & 0 & 0.90 & 0 & 0.90 & 0 ±0 & 0.90 ±0.00 \\
stack\_bowls & 18 & 21.30 & 14 & 17.00 & 12 & 15.00 & 15 ±3 & 17.77 ±3.15 \\
store\_laptop\_and\_headphones & 0 & 0.40 & 0 & 1.60 & 0 & 3.60 & 0 ±0 & 1.87 ±1.60 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 8.20 & 0 & 0.40 & 4 & 5.00 & 1 ±2 & 4.53 ±3.90 \\
deposit\_coin & 0 & 0.00 & 0 & 0.80 & 0 & 0.80 & 0 ±0 & 0.53 ±0.40 \\
fasten\_screws & 0 & 0.00 & 0 & 0.40 & 0 & 0.80 & 0 ±0 & 0.40 ±0.40 \\
insert\_key & 0 & 3.90 & 0 & 7.50 & 0 & 9.00 & 0 ±0 & 6.80 ±2.55 \\
insert\_tubes & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 4 & 4.00 & 8 & 8.00 & 12 & 12.00 & 8 ±4 & 8.00 ±4.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.90 & 0 & 2.70 & 0 & 1.50 & 0 ±0 & 1.70 ±0.90 \\
fill\_egg\_holder & 0 & 2.70 & 0 & 2.60 & 0 & 2.70 & 0 ±0 & 2.67 ±0.05 \\
fill\_pen\_holder & 0 & 1.20 & 0 & 3.20 & 0 & 3.90 & 0 ±0 & 2.77 ±1.35 \\
make\_kong & 4 & 4.00 & 0 & 0.00 & 0 & 0.00 & 1 ±2 & 1.33 ±2.00 \\
organize\_table & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 1.60 & 0 & 0.20 & 0 & 1.00 & 0 ±0 & 0.93 ±0.70 \\
put\_bottles\_into\_dustbin & 8 & 25.60 & 28 & 46.90 & 24 & 42.80 & 20 ±10 & 38.43 ±10.65 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.40 & 0 & 0.40 & 0 & 0.70 & 0 ±0 & 0.50 ±0.15 \\
match\_and\_pick\_from\_conveyor & 6 & 6.00 & 8 & 8.00 & 10 & 10.00 & 8 ±2 & 8.00 ±2.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.60 & 0 & 0.20 & 0 & 0.20 & 0 ±0 & 0.33 ±0.20 \\
general\_pickup & 2 & 2.00 & 2 & 2.00 & 4 & 4.00 & 3 ±1 & 2.67 ±1.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.27 ±0.20 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 1.1 & 2.22 & 1.9 & 3.22 & 2.0 & 3.47 & 2 ±0 & 2.97 ±0.62 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Pi-05}
\label{part:pi_05}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.80 & 0 & 0.90 & 0 & 2.00 & 0 ±0 & 1.23 ±0.60 \\
fold\_clothes & 8 & 16.40 & 8 & 18.80 & 10 & 24.80 & 9 ±1 & 20.00 ±4.20 \\
hang\_mugs & 0 & 2.70 & 0 & 4.90 & 0 & 4.30 & 0 ±0 & 3.97 ±1.10 \\
make\_toast & 0 & 3.00 & 2 & 7.50 & 2 & 5.50 & 1 ±1 & 5.33 ±2.25 \\
pack\_objects\_into\_box & 2 & 14.40 & 2 & 11.70 & 4 & 18.80 & 3 ±1 & 14.97 ±3.55 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 12 & 12.00 & 16 & 16.00 & 9 ±8 & 9.33 ±8.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 2 & 2.00 & 6 & 6.00 & 3 ±3 & 2.67 ±3.00 \\
stack\_blocks & 2 & 5.60 & 6 & 10.80 & 14 & 17.00 & 7 ±6 & 11.13 ±5.70 \\
stack\_bowls & 42 & 46.50 & 36 & 42.30 & 48 & 53.70 & 42 ±6 & 47.50 ±5.70 \\
store\_laptop\_and\_headphones & 0 & 8.00 & 0 & 2.80 & 2 & 8.00 & 1 ±1 & 6.27 ±2.60 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 3.40 & 8 & 20.80 & 34 & 46.20 & 14 ±17 & 23.47 ±21.40 \\
deposit\_coin & 0 & 0.40 & 2 & 2.80 & 0 & 2.00 & 1 ±1 & 1.73 ±1.20 \\
fasten\_screws & 0 & 4.00 & 0 & 8.20 & 0 & 6.20 & 0 ±0 & 6.13 ±2.10 \\
insert\_key & 0 & 10.50 & 0 & 11.40 & 0 & 11.10 & 0 ±0 & 11.00 ±0.45 \\
insert\_tubes & 0 & 7.20 & 2 & 9.20 & 0 & 12.00 & 1 ±1 & 9.47 ±2.40 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 4 & 4.00 & 8 & 8.00 & 18 & 18.00 & 10 ±7 & 10.00 ±7.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 14 & 22.90 & 10 & 21.50 & 20 & 33.10 & 15 ±5 & 25.83 ±5.80 \\
fill\_egg\_holder & 0 & 3.10 & 0 & 1.40 & 0 & 2.30 & 0 ±0 & 2.27 ±0.85 \\
fill\_pen\_holder & 2 & 16.60 & 0 & 11.50 & 10 & 30.10 & 4 ±5 & 19.40 ±9.30 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 27.50 & 2 & 26.50 & 0 & 29.00 & 1 ±1 & 27.67 ±1.25 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.20 & 0 & 0.00 & 0 & 0.20 & 0 ±0 & 0.13 ±0.10 \\
put\_bottles\_into\_dustbin & 46 & 63.40 & 54 & 70.00 & 78 & 85.90 & 59 ±16 & 73.10 ±11.25 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.30 & 0 & 1.50 & 0 & 1.30 & 0 ±0 & 1.03 ±0.60 \\
imitate\_sorting\_sequence & 0 & 1.00 & 0 & 0.80 & 0 & 1.30 & 0 ±0 & 1.03 ±0.25 \\
match\_and\_pick\_from\_conveyor & 6 & 6.00 & 10 & 10.00 & 4 & 4.00 & 7 ±3 & 6.67 ±3.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 2 & 2.00 & 1 ±1 & 0.67 ±1.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.40 & 0 & 1.20 & 0 & 1.40 & 0 ±0 & 1.00 ±0.50 \\
general\_pickup & 4 & 4.00 & 8 & 8.00 & 12 & 12.00 & 8 ±4 & 8.00 ±4.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.40 & 0 & 2.40 & 2 & 3.20 & 1 ±1 & 2.00 ±1.40 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.50 & 0 ±0 & 0.17 ±0.25 \\
\hline
\textbf{Avg} & 3.1 & 6.49 & 4.1 & 7.83 & 6.7 & 10.90 & 5 ±2 & 8.41 ±2.20 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{RDT-1B}
\label{part:rdt_1b}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number &  &  &  &  &  &  &  &  \\
fold\_clothes &  &  &  &  &  &  &  &  \\
hang\_mugs &  &  &  &  &  &  &  &  \\
make\_toast &  &  &  &  &  &  &  &  \\
pack\_objects\_into\_box &  &  &  &  &  &  &  &  \\
pour\_liquid\_into\_cup &  &  &  &  &  &  &  &  \\
push\_T &  &  &  &  &  &  &  &  \\
sort\_nesting\_dolls\_by\_size &  &  &  &  &  &  &  &  \\
stack\_blocks &  &  &  &  &  &  &  &  \\
stack\_bowls &  &  &  &  &  &  &  &  \\
store\_laptop\_and\_headphones &  &  &  &  &  &  &  &  \\
sweep\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower &  &  &  &  &  &  &  &  \\
deposit\_coin &  &  &  &  &  &  &  &  \\
fasten\_screws &  &  &  &  &  &  &  &  \\
insert\_key &  &  &  &  &  &  &  &  \\
insert\_tubes &  &  &  &  &  &  &  &  \\
play\_Xylophone &  &  &  &  &  &  &  &  \\
plug\_in\_charger &  &  &  &  &  &  &  &  \\
pour\_balls\_into\_vase &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects &  &  &  &  &  &  &  &  \\
fill\_egg\_holder &  &  &  &  &  &  &  &  \\
fill\_pen\_holder &  &  &  &  &  &  &  &  \\
make\_kong &  &  &  &  &  &  &  &  \\
organize\_table &  &  &  &  &  &  &  &  \\
play\_stacking\_toy &  &  &  &  &  &  &  &  \\
play\_tic\_tac\_toe &  &  &  &  &  &  &  &  \\
put\_bottles\_into\_dustbin &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks &  &  &  &  &  &  &  &  \\
imitate\_sorting\_sequence &  &  &  &  &  &  &  &  \\
match\_and\_pick\_from\_conveyor &  &  &  &  &  &  &  &  \\
press\_by\_number &  &  &  &  &  &  &  &  \\
swap\_T &  &  &  &  &  &  &  &  \\
swap\_blocks &  &  &  &  &  &  &  &  \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image &  &  &  &  &  &  &  &  \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{SmolVLA}
\label{part:smolvla}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.10 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.03 ±0.05 \\
fold\_clothes & 8 & 9.20 & 4 & 4.40 & 10 & 11.20 & 7 ±3 & 8.27 ±3.40 \\
hang\_mugs & 0 & 0.60 & 0 & 0.30 & 0 & 1.10 & 0 ±0 & 0.67 ±0.40 \\
make\_toast & 0 & 1.50 & 0 & 1.00 & 0 & 1.50 & 0 ±0 & 1.33 ±0.25 \\
pack\_objects\_into\_box &  &  &  &  &  &  &  &  \\
pour\_liquid\_into\_cup & 2 & 2.00 & 4 & 4.00 & 10 & 10.00 & 5 ±4 & 5.33 ±4.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.30 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.10 ±0.15 \\
stack\_bowls & 2 & 4.70 &  &  & 0 & 1.20 &  &  \\
store\_laptop\_and\_headphones & 0 & 0.80 & 0 & 0.80 & 0 & 0.40 & 0 ±0 & 0.67 ±0.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 1.80 & 2 & 9.00 & 0 & 6.40 & 1 ±1 & 5.73 ±3.60 \\
deposit\_coin & 0 & 0.40 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.40 ±0.00 \\
fasten\_screws & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_key & 0 & 7.20 & 0 & 6.30 & 0 & 5.70 & 0 ±0 & 6.40 ±0.75 \\
insert\_tubes & 2 & 8.80 & 0 & 8.00 & 0 & 10.40 & 1 ±1 & 9.07 ±1.20 \\
play\_Xylophone & 2 & 2.00 & 0 & 0.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.30 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.10 ±0.15 \\
fill\_egg\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
fill\_pen\_holder & 0 & 1.90 & 0 & 1.70 & 0 & 0.20 & 0 ±0 & 1.27 ±0.85 \\
make\_kong & 2 & 2.00 & 4 & 4.00 & 0 & 0.00 & 2 ±2 & 2.00 ±2.00 \\
organize\_table & 0 & 2.00 & 0 & 2.00 & 0 & 0.50 & 0 ±0 & 1.50 ±0.75 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 1.40 & 0 & 0.80 & 0 & 0.80 & 0 ±0 & 1.00 ±0.30 \\
put\_bottles\_into\_dustbin & 0 & 5.40 & 0 & 2.60 & 0 & 3.20 & 0 ±0 & 3.73 ±1.40 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 6 & 11.10 & 6 & 12.00 & 2 & 7.00 & 5 ±2 & 10.03 ±2.50 \\
imitate\_sorting\_sequence & 0 & 0.00 & 0 & 0.10 & 0 & 0.10 & 0 ±0 & 0.07 ±0.05 \\
match\_and\_pick\_from\_conveyor & 12 & 12.00 & 4 & 4.00 & 14 & 14.00 & 10 ±5 & 10.00 ±5.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks &  &  &  &  &  &  &  &  \\
classify\_objects\_by\_language &  &  &  &  &  &  &  &  \\
general\_pickup &  &  &  &  &  &  &  &  \\
pick\_from\_conveyor\_by\_image &  &  &  &  &  &  &  &  \\
pour\_by\_language &  &  &  &  &  &  &  &  \\
solve\_equation &  &  &  &  &  &  &  &  \\
stack\_blocks\_by\_language &  &  &  &  &  &  &  &  \\
store\_tools\_in\_toolbox &  &  &  &  &  &  &  &  \\
\hline
\textbf{Avg} & 1.1 & 2.29 & 0.8 & 1.98 & 1.1 & 2.26 & 1 ±0 & 2.18 ±0.15 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Spirit\_v15}
\label{part:spirit_v15}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.20 & 0 ±0 & 0.07 ±0.10 \\
fold\_clothes & 0 & 0.00 & 0 & 1.60 & 0 & 1.20 & 0 ±0 & 0.93 ±0.80 \\
hang\_mugs & 0 & 0.00 & 0 & 1.20 & 0 & 0.60 & 0 ±0 & 0.60 ±0.60 \\
make\_toast & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pack\_objects\_into\_box & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_bowls & 10 & 11.80 & 4 & 6.40 & 4 & 5.80 & 6 ±3 & 8.00 ±3.00 \\
store\_laptop\_and\_headphones & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
deposit\_coin & 0 & 0.00 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
fasten\_screws & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_key & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_tubes & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_egg\_holder & 0 & 0.00 & 0 & 0.40 & 0 & 0.40 & 0 ±0 & 0.27 ±0.20 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 0.50 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.17 ±0.25 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.40 & 0 & 0.60 & 0 & 0.20 & 0 ±0 & 0.40 ±0.20 \\
put\_bottles\_into\_dustbin & 0 & 0.00 & 0 & 0.20 & 0 & 0.00 & 0 ±0 & 0.07 ±0.10 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
match\_and\_pick\_from\_conveyor & 2 & 2.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 1.33 ±1.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.3 & 0.35 & 0.1 & 0.30 & 0.1 & 0.21 & 0 ±0 & 0.29 ±0.07 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{TinyVLA}
\label{part:tinyvla}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fold\_clothes & 0 & 0.00 & 0 & 0.40 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
hang\_mugs & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_toast & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pack\_objects\_into\_box & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
pour\_liquid\_into\_cup & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_bowls & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_laptop\_and\_headphones & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
deposit\_coin & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
fasten\_screws & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
insert\_key & 0 & 0.00 & 0 & 0.00 & 0 & 0.30 & 0 ±0 & 0.10 ±0.15 \\
insert\_tubes & 0 & 0.00 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.13 ±0.20 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_egg\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
fill\_pen\_holder & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
make\_kong & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
organize\_table & 0 & 3.00 & 0 & 3.00 & 0 & 1.00 & 0 ±0 & 2.33 ±1.00 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 0.40 & 0 & 0.40 & 0 & 0.60 & 0 ±0 & 0.47 ±0.10 \\
put\_bottles\_into\_dustbin & 0 & 1.80 & 0 & 2.10 & 0 & 3.80 & 0 ±0 & 2.57 ±1.00 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
imitate\_sorting\_sequence & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
match\_and\_pick\_from\_conveyor & 0 & 0.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
general\_pickup & 0 & 0.00 & 6 & 6.00 & 0 & 0.00 & 2 ±3 & 2.00 ±3.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 0.0 & 0.12 & 0.2 & 0.33 & 0.0 & 0.17 & 0 ±0 & 0.21 ±0.10 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{X\_VLA}
\label{part:x_vla}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 2.40 & 0 & 2.70 & 0 & 2.30 & 0 ±0 & 2.47 ±0.20 \\
fold\_clothes & 14 & 22.40 & 36 & 40.80 & 16 & 23.20 & 22 ±11 & 28.80 ±9.20 \\
hang\_mugs & 0 & 6.60 & 0 & 6.50 & 0 & 7.80 & 0 ±0 & 6.97 ±0.65 \\
make\_toast & 2 & 4.50 & 0 & 4.50 & 2 & 5.00 & 1 ±1 & 4.67 ±0.25 \\
pack\_objects\_into\_box & 0 & 7.30 & 2 & 9.80 & 0 & 5.60 & 1 ±1 & 7.57 ±2.10 \\
pour\_liquid\_into\_cup & 16 & 16.00 & 14 & 14.00 & 10 & 10.00 & 13 ±3 & 13.33 ±3.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 4 & 4.00 & 12 & 12.00 & 2 & 2.00 & 6 ±5 & 6.00 ±5.00 \\
stack\_blocks & 4 & 8.80 & 10 & 14.20 & 8 & 11.30 & 7 ±3 & 11.43 ±2.70 \\
stack\_bowls & 34 & 38.20 & 24 & 28.80 & 20 & 24.20 & 26 ±7 & 30.40 ±7.00 \\
store\_laptop\_and\_headphones & 2 & 11.60 & 6 & 16.00 & 6 & 14.80 & 5 ±2 & 14.13 ±2.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 60 & 70.00 & 58 & 67.00 & 42 & 52.60 & 53 ±9 & 63.20 ±8.70 \\
deposit\_coin & 0 & 5.60 & 4 & 12.40 & 2 & 9.20 & 2 ±2 & 9.07 ±3.40 \\
fasten\_screws & 0 & 6.80 & 0 & 7.20 & 0 & 6.80 & 0 ±0 & 6.93 ±0.20 \\
insert\_key & 0 & 11.10 & 0 & 11.40 & 0 & 14.40 & 0 ±0 & 12.30 ±1.65 \\
insert\_tubes & 50 & 64.40 & 30 & 43.60 & 12 & 27.20 & 31 ±19 & 45.07 ±18.60 \\
play\_Xylophone & 0 & 0.00 & 2 & 2.00 & 2 & 2.00 & 1 ±1 & 1.33 ±1.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 10 & 10.00 & 10 & 10.00 & 6 & 6.00 & 9 ±2 & 8.67 ±2.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 5.20 & 2 & 5.80 & 0 & 2.70 & 1 ±1 & 4.57 ±1.55 \\
fill\_egg\_holder & 0 & 0.40 & 0 & 0.20 & 0 & 0.40 & 0 ±0 & 0.33 ±0.10 \\
fill\_pen\_holder & 2 & 16.50 & 2 & 12.20 & 0 & 7.80 & 1 ±1 & 12.17 ±4.35 \\
make\_kong & 10 & 10.00 & 2 & 2.00 & 14 & 14.00 & 9 ±6 & 8.67 ±6.00 \\
organize\_table & 2 & 20.00 & 6 & 26.00 & 4 & 15.50 & 4 ±2 & 20.50 ±5.25 \\
play\_stacking\_toy & 0 & 0.20 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.07 ±0.10 \\
play\_tic\_tac\_toe & 0 & 2.60 & 2 & 18.60 & 2 & 13.90 & 1 ±1 & 11.70 ±8.00 \\
put\_bottles\_into\_dustbin & 60 & 73.30 & 62 & 75.10 & 64 & 74.30 & 62 ±2 & 74.23 ±0.90 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 10 & 18.40 & 18 & 25.20 & 18 & 24.10 & 15 ±4 & 22.57 ±3.40 \\
imitate\_sorting\_sequence & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
match\_and\_pick\_from\_conveyor & 6 & 6.00 & 8 & 8.00 & 4 & 4.00 & 6 ±2 & 6.00 ±2.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.00 & 0 & 0.60 & 0 & 0.20 & 0 ±0 & 0.27 ±0.30 \\
general\_pickup & 2 & 2.00 & 6 & 6.00 & 4 & 4.00 & 4 ±2 & 4.00 ±2.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.40 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 6.9 & 10.59 & 7.5 & 11.49 & 5.7 & 9.17 & 7 ±1 & 10.42 ±1.16 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{X\_WAM}
\label{part:x_wam}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 1.60 & 0 & 2.40 & 0 & 1.10 & 0 ±0 & 1.70 ±0.65 \\
fold\_clothes & 14 & 20.40 & 14 & 19.60 & 8 & 15.60 & 12 ±3 & 18.53 ±2.40 \\
hang\_mugs & 2 & 6.30 & 2 & 8.50 & 0 & 5.80 & 1 ±1 & 6.87 ±1.35 \\
make\_toast & 2 & 12.00 & 0 & 4.00 & 0 & 4.50 & 1 ±1 & 6.83 ±4.00 \\
pack\_objects\_into\_box & 0 & 12.00 & 0 & 11.60 & 0 & 12.20 & 0 ±0 & 11.93 ±0.30 \\
pour\_liquid\_into\_cup & 2 & 2.00 & 12 & 12.00 & 4 & 4.00 & 6 ±5 & 6.00 ±5.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 4 & 4.00 & 0 & 0.00 & 2 & 2.00 & 2 ±2 & 2.00 ±2.00 \\
stack\_blocks & 2 & 7.70 & 0 & 6.30 & 0 & 6.00 & 1 ±1 & 6.67 ±0.85 \\
stack\_bowls & 10 & 18.40 & 20 & 25.70 & 20 & 26.30 & 17 ±5 & 23.47 ±3.95 \\
store\_laptop\_and\_headphones & 0 & 5.20 & 2 & 5.60 & 0 & 3.20 & 1 ±1 & 4.67 ±1.20 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 2 & 4.80 & 4 & 7.40 & 0 & 3.60 & 2 ±2 & 5.27 ±1.90 \\
deposit\_coin & 0 & 2.40 & 0 & 2.80 & 0 & 4.00 & 0 ±0 & 3.07 ±0.80 \\
fasten\_screws & 2 & 13.60 & 0 & 14.60 & 0 & 11.40 & 1 ±1 & 13.20 ±1.60 \\
insert\_key & 0 & 6.30 & 0 & 6.30 & 0 & 5.70 & 0 ±0 & 6.10 ±0.30 \\
insert\_tubes & 2 & 16.00 & 4 & 17.20 & 2 & 17.20 & 3 ±1 & 16.80 ±0.60 \\
play\_Xylophone & 4 & 4.00 & 4 & 4.00 & 12 & 12.00 & 7 ±4 & 6.67 ±4.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 4 & 4.00 & 2 & 2.00 & 2 & 2.00 & 3 ±1 & 2.67 ±1.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 3.30 & 2 & 6.90 & 0 & 8.20 & 1 ±1 & 6.13 ±2.45 \\
fill\_egg\_holder & 0 & 4.90 & 0 & 1.60 & 0 & 3.50 & 0 ±0 & 3.33 ±1.65 \\
fill\_pen\_holder & 0 & 7.30 & 0 & 7.90 & 0 & 6.10 & 0 ±0 & 7.10 ±0.90 \\
make\_kong & 8 & 8.00 & 2 & 2.00 & 0 & 0.00 & 3 ±4 & 3.33 ±4.00 \\
organize\_table & 0 & 25.50 & 0 & 28.50 & 0 & 32.50 & 0 ±0 & 28.83 ±3.50 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.20 & 0 ±0 & 0.07 ±0.10 \\
play\_tic\_tac\_toe & 0 & 9.60 & 0 & 16.00 & 0 & 7.60 & 0 ±0 & 11.07 ±4.20 \\
put\_bottles\_into\_dustbin & 70 & 81.70 & 72 & 81.70 & 64 & 76.30 & 69 ±4 & 79.90 ±2.70 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 4 & 13.00 & 8 & 17.70 & 2 & 10.60 & 5 ±3 & 13.77 ±3.55 \\
imitate\_sorting\_sequence & 0 & 0.70 & 0 & 0.40 & 0 & 1.30 & 0 ±0 & 0.80 ±0.45 \\
match\_and\_pick\_from\_conveyor & 16 & 16.00 & 34 & 34.00 & 16 & 16.00 & 22 ±9 & 22.00 ±9.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 2 & 2.00 & 1 ±1 & 0.67 ±1.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 2 & 2.00 & 1 ±1 & 0.67 ±1.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 1.00 & 0 & 1.40 & 0 & 0.80 & 0 ±0 & 1.07 ±0.30 \\
general\_pickup & 0 & 0.00 & 2 & 2.00 & 2 & 2.00 & 1 ±1 & 1.33 ±1.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 2 & 2.00 & 1 ±1 & 0.67 ±1.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 1.60 & 0 & 1.60 & 0 & 0.80 & 0 ±0 & 1.33 ±0.40 \\
store\_tools\_in\_toolbox & 0 & 0.50 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.17 ±0.25 \\
\hline
\textbf{Avg} & 3.5 & 7.47 & 4.4 & 8.37 & 3.3 & 7.35 & 4 ±1 & 7.73 ±0.51 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{Xiaomi\_Robotics\_0}
\label{part:xiaomi_robotics_0}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 1.20 & 0 & 0.70 & 0 & 0.80 & 0 ±0 & 0.90 ±0.25 \\
fold\_clothes & 22 & 24.40 & 22 & 26.00 & 16 & 18.00 & 20 ±3 & 22.80 ±4.00 \\
hang\_mugs & 0 & 2.00 & 0 & 3.20 & 0 & 4.70 & 0 ±0 & 3.30 ±1.35 \\
make\_toast & 0 & 1.00 & 0 & 3.00 & 0 & 1.00 & 0 ±0 & 1.67 ±1.00 \\
pack\_objects\_into\_box & 0 & 3.50 & 0 & 3.00 & 0 & 3.80 & 0 ±0 & 3.43 ±0.40 \\
pour\_liquid\_into\_cup & 8 & 8.00 & 18 & 18.00 & 20 & 20.00 & 15 ±6 & 15.33 ±6.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 0 & 0.00 & 2 & 2.00 & 1 ±1 & 0.67 ±1.00 \\
stack\_blocks & 2 & 3.80 & 6 & 8.40 & 2 & 4.40 & 3 ±2 & 5.53 ±2.30 \\
stack\_bowls & 32 & 36.50 & 24 & 27.00 & 18 & 22.20 & 25 ±7 & 28.57 ±7.15 \\
store\_laptop\_and\_headphones & 4 & 8.40 & 0 & 2.40 & 4 & 10.00 & 3 ±2 & 6.93 ±3.80 \\
sweep\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 6 & 6.60 & 8 & 10.80 & 8 & 11.60 & 7 ±1 & 9.67 ±2.50 \\
deposit\_coin & 0 & 4.00 & 0 & 2.80 & 0 & 4.00 & 0 ±0 & 3.60 ±0.60 \\
fasten\_screws & 0 & 1.60 & 0 & 3.80 & 0 & 7.40 & 0 ±0 & 4.27 ±2.90 \\
insert\_key & 0 & 5.70 & 0 & 9.00 & 0 & 10.80 & 0 ±0 & 8.50 ±2.55 \\
insert\_tubes & 2 & 12.00 & 0 & 9.60 & 12 & 28.40 & 5 ±6 & 16.67 ±9.40 \\
play\_Xylophone & 4 & 4.00 & 0 & 0.00 & 4 & 4.00 & 3 ±2 & 2.67 ±2.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 18 & 18.00 & 24 & 24.00 & 24 & 24.00 & 22 ±3 & 22.00 ±3.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 3.50 & 2 & 3.50 & 0 & 3.60 & 1 ±1 & 3.53 ±0.05 \\
fill\_egg\_holder & 0 & 1.60 & 0 & 1.60 & 0 & 1.30 & 0 ±0 & 1.50 ±0.15 \\
fill\_pen\_holder & 2 & 16.30 & 0 & 12.40 & 4 & 15.90 & 2 ±2 & 14.87 ±1.95 \\
make\_kong & 18 & 18.00 & 14 & 14.00 & 6 & 6.00 & 13 ±6 & 12.67 ±6.00 \\
organize\_table & 0 & 17.00 & 0 & 17.00 & 4 & 15.50 & 1 ±2 & 16.50 ±0.75 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 3.40 & 0 & 5.80 & 0 & 6.60 & 0 ±0 & 5.27 ±1.60 \\
put\_bottles\_into\_dustbin & 38 & 52.60 & 54 & 65.60 & 24 & 43.10 & 39 ±15 & 53.77 ±11.25 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 6 & 13.30 & 0 & 8.30 & 10 & 16.80 & 5 ±5 & 12.80 ±4.25 \\
imitate\_sorting\_sequence & 0 & 1.10 & 0 & 0.30 & 0 & 1.50 & 0 ±0 & 0.97 ±0.60 \\
match\_and\_pick\_from\_conveyor & 20 & 20.00 & 16 & 16.00 & 14 & 14.00 & 17 ±3 & 16.67 ±3.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.20 & 0 & 0.40 & 0 & 0.20 & 0 ±0 & 0.27 ±0.10 \\
general\_pickup & 4 & 4.00 & 0 & 0.00 & 0 & 0.00 & 1 ±2 & 1.33 ±2.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 0.40 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.13 ±0.20 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 4.4 & 6.95 & 4.5 & 7.06 & 4.1 & 7.18 & 4 ±0 & 7.07 ±0.11 \\
\hline
\end{tabular}
}
\end{table}
% =========================================================
\subsection{starVLA}
\label{part:starvla}

\begin{table}[H]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
Task & S0 SR & S0 Score & S1 SR & S1 Score & S2 SR & S2 Score & Avg SR & Avg Score \\
\hline
\multicolumn{9}{l}{\textbf{Generalization}} \\
arrange\_largest\_number & 0 & 0.80 & 0 & 0.50 & 0 & 0.60 & 0 ±0 & 0.63 ±0.15 \\
fold\_clothes & 6 & 10.40 & 10 & 12.80 & 8 & 12.80 & 8 ±2 & 12.00 ±1.20 \\
hang\_mugs & 0 & 1.50 & 0 & 3.90 & 0 & 2.30 & 0 ±0 & 2.57 ±1.20 \\
make\_toast & 0 & 1.00 & 0 & 1.50 & 0 & 3.00 & 0 ±0 & 1.83 ±1.00 \\
pack\_objects\_into\_box & 0 & 2.60 & 0 & 4.20 & 4 & 6.90 & 1 ±2 & 4.57 ±2.15 \\
pour\_liquid\_into\_cup & 14 & 14.00 & 4 & 4.00 & 10 & 10.00 & 9 ±5 & 9.33 ±5.00 \\
push\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
sort\_nesting\_dolls\_by\_size & 0 & 0.00 & 2 & 2.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
stack\_blocks & 6 & 7.50 & 0 & 1.80 & 2 & 3.20 & 3 ±3 & 4.17 ±2.85 \\
stack\_bowls & 6 & 9.60 & 8 & 11.60 & 2 & 3.50 & 5 ±3 & 8.23 ±4.05 \\
store\_laptop\_and\_headphones & 0 & 2.80 & 0 & 2.40 & 0 & 2.40 & 0 ±0 & 2.53 ±0.20 \\
sweep\_blocks & 2 & 2.00 & 0 & 0.00 & 0 & 0.00 & 1 ±1 & 0.67 ±1.00 \\
\hline
\multicolumn{9}{l}{\textbf{Precision}} \\
build\_tower & 40 & 51.40 & 16 & 37.00 & 22 & 37.80 & 26 ±12 & 42.07 ±7.20 \\
deposit\_coin & 2 & 6.00 & 0 & 3.20 & 2 & 6.40 & 1 ±1 & 5.20 ±1.60 \\
fasten\_screws & 0 & 1.60 & 0 & 1.20 & 0 & 2.00 & 0 ±0 & 1.60 ±0.40 \\
insert\_key & 0 & 10.50 & 0 & 11.70 & 0 & 12.30 & 0 ±0 & 11.50 ±0.90 \\
insert\_tubes & 0 & 12.00 & 2 & 12.80 & 4 & 15.60 & 2 ±2 & 13.47 ±1.80 \\
play\_Xylophone & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
plug\_in\_charger & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_balls\_into\_vase & 2 & 2.00 & 8 & 8.00 & 6 & 6.00 & 5 ±3 & 5.33 ±3.00 \\
\hline
\multicolumn{9}{l}{\textbf{Long-Horizon}} \\
classify\_objects & 0 & 3.50 & 0 & 3.40 & 0 & 1.80 & 0 ±0 & 2.90 ±0.85 \\
fill\_egg\_holder & 0 & 1.00 & 0 & 1.60 & 0 & 0.80 & 0 ±0 & 1.13 ±0.40 \\
fill\_pen\_holder & 6 & 19.10 & 10 & 20.70 & 2 & 12.90 & 6 ±4 & 17.57 ±3.90 \\
make\_kong & 22 & 22.00 & 30 & 30.00 & 2 & 2.00 & 18 ±14 & 18.00 ±14.00 \\
organize\_table & 0 & 24.00 & 0 & 27.00 & 0 & 16.00 & 0 ±0 & 22.33 ±5.50 \\
play\_stacking\_toy & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
play\_tic\_tac\_toe & 0 & 2.60 & 0 & 1.00 & 0 & 3.60 & 0 ±0 & 2.40 ±1.30 \\
put\_bottles\_into\_dustbin & 24 & 43.80 & 28 & 51.80 & 32 & 51.10 & 28 ±4 & 48.90 ±4.00 \\
\hline
\multicolumn{9}{l}{\textbf{Memory}} \\
cover\_blocks & 12 & 19.50 & 6 & 10.30 & 12 & 14.40 & 10 ±3 & 14.73 ±4.60 \\
imitate\_sorting\_sequence & 0 & 0.50 & 0 & 0.60 & 0 & 0.80 & 0 ±0 & 0.63 ±0.15 \\
match\_and\_pick\_from\_conveyor & 10 & 10.00 & 4 & 4.00 & 0 & 0.00 & 5 ±5 & 4.67 ±5.00 \\
press\_by\_number & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_T & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
swap\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\multicolumn{9}{l}{\textbf{Open}} \\
align\_blocks & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
classify\_objects\_by\_language & 0 & 0.20 & 0 & 0.20 & 0 & 0.20 & 0 ±0 & 0.20 ±0.00 \\
general\_pickup & 6 & 6.00 & 2 & 2.00 & 6 & 6.00 & 5 ±2 & 4.67 ±2.00 \\
pick\_from\_conveyor\_by\_image & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
pour\_by\_language & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
solve\_equation & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
stack\_blocks\_by\_language & 0 & 1.20 & 0 & 0.00 & 0 & 0.40 & 0 ±0 & 0.53 ±0.60 \\
store\_tools\_in\_toolbox & 0 & 0.00 & 0 & 0.00 & 0 & 0.00 & 0 ±0 & 0.00 ±0.00 \\
\hline
\textbf{Avg} & 3.8 & 6.88 & 3.1 & 6.46 & 2.7 & 5.59 & 3 ±1 & 6.31 ±0.65 \\
\hline
\end{tabular}
}
\end{table}

==> table/evaluation_speed.tex <==
\begin{table*}[!ht]
\centering
\caption{\textbf{Evaluation Speed}. 640$\times$480 resolution.}
\label{tab:benchmark_eval_efficiency}
\begingroup
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\definecolor{bestblue}{RGB}{210,243,247}
\newcommand{\thickline}{\noalign{\vspace{0.25em}\hrule height 1.2pt\vspace{0.25em}}}
\newcommand{\thicksep}{%
\vspace{0.25em}
\noindent\rule{\textwidth}{1.2pt}
\vspace{0.25em}
}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\thickline
\textbf{Benchmark} & \textbf{Platform} & \textbf{Render} &  \textbf{Physics} & \textbf{Compute} & \textbf{HP\footnote{HP indicates Heterogeneous Parallelization}} & \textbf{Tasks} & \textbf{Frames} & \textbf{Time} & \textbf{100 Frame Freq.}\\
\midrule
RoboTwin 1.0 & SAPIEN \\
RoboTwin 2.0 & SAPIEN \\
LIBERO  & Mujoco \\
CALVIN & \\
RLBench & \\
RoboCasa & \\
SimplerEnv & \\
VLABench & \\
BEHAVIOR 1K \\
RoboSuite & Mujoco \\
Meta-World & Mujoco \\
EBench & IsaacSim \\
\midrule
RoboDojo (ours) & IsaacSim & & PhysX & GPU\\
\thickline

\end{tabular}
}
\endgroup
\end{table*}

==> table/real_consistency.tex <==
\begin{table*}[t]
\centering
\caption{Real-world evaluation consistency across three repeated runs. We report the standard deviation of success rate and score across R1--R3. Scores are multiplied by 100 for readability.}
\label{tab:real_world_consistency_std}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Task}
& \multicolumn{2}{c}{$\pi_{0.5}$}
& \multicolumn{2}{c}{GalaxeaVLA}
& \multicolumn{2}{c}{InternVLA-A1} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& Std. SR & Std. Score
& Std. SR & Std. Score
& Std. SR & Std. Score \\
\midrule
\texttt{connect\_charger} & 0.0\% & 0.0 & 0.0\% & 0.0 & 0.0\% & 0.0 \\
\texttt{stack\_bowls} & 5.8\% & 4.0 & 15.3\% & 16.6 & 5.8\% & 3.5 \\
\texttt{stack\_and\_cover\_blocks} & 5.8\% & 5.8 & 0.0\% & 0.0 & 0.0\% & 0.0 \\
\texttt{fill\_pen\_holder} & 10.0\% & 1.2 & 5.8\% & 11.7 & 0.0\% & 3.5 \\
\texttt{stand\_up\_bottles} & 5.8\% & 6.6 & 0.0\% & 7.8 & 15.3\% & 9.8 \\
\texttt{put\_objects\_into\_basket} & 5.8\% & 5.8 & 5.8\% & 5.8 & 5.8\% & 5.8 \\
\texttt{hang\_mugs} & 0.0\% & 1.2 & 0.0\% & 2.3 & 0.0\% & 2.3 \\
\texttt{pack\_objects\_into\_backpack} & 5.8\% & 3.5 & 0.0\% & 1.7 & 0.0\% & 6.5 \\
\texttt{sweep\_blocks} & 5.8\% & 5.8 & 5.8\% & 5.8 & 0.0\% & 0.0 \\
\texttt{disassemble\_LEGO} & 5.8\% & 4.6 & 0.0\% & 1.2 & 0.0\% & 0.0 \\
\texttt{classify\_objects} & 0.0\% & 2.3 & 0.0\% & 0.0 & 0.0\% & 0.0 \\
\texttt{cap\_pen} & 0.0\% & 2.0 & 0.0\% & 2.3 & 0.0\% & 2.0 \\
\texttt{pack\_and\_pour\_fruit} & 5.8\% & 3.1 & 0.0\% & 3.5 & 0.0\% & 10.0 \\
\texttt{store\_in\_safe} & 23.1\% & 12.9 & 11.5\% & 13.9 & 17.3\% & 10.4 \\
\texttt{make\_food} & 5.8\% & 5.1 & 0.0\% & 1.7 & 0.0\% & 0.0 \\
\texttt{insert\_tubes} & 5.8\% & 6.4 & 0.0\% & 8.4 & 0.0\% & 4.6 \\
\texttt{cover\_blocks} & 5.8\% & 4.6 & 0.0\% & 0.3 & 0.0\% & 0.0 \\
\texttt{make\_bread} & 0.0\% & 0.0 & 0.0\% & 0.0 & 0.0\% & 0.0 \\
\midrule
\textbf{Average} & \textbf{1.0\%} & \textbf{0.5} & \textbf{1.2\%} & \textbf{1.0} & \textbf{1.3\%} & \textbf{1.2} \\
\bottomrule
\end{tabular}
\end{table*}
